The LOFAR Two-metre Sky Survey: The nature of the faint source population and SFR-radio luminosity relation using Prospector

Spectral energy distribution (SED) fitting has been extensively used to determine the nature of the faint radio source population. Recent efforts have combined fits from multiple SED-fitting codes to account for the host galaxy and any active nucleus that may be present. We show that it is possible to produce similar-quality classifications using a single energy-balance SED fitting code, Prospector, to model up to 26 bands of UV$-$far-infrared aperture-matched photometry for $\sim$31,000 sources in the ELAIS-N1 field from the LOFAR Two-Metre Sky Survey (LoTSS) Deep fields first data release. One of a new generation of SED-fitting codes, Prospector accounts for potential contributions from radiative active galactic nuclei (AGN) when estimating galaxy properties, including star formation rates (SFRs) derived using non-parametric star formation histories. Combining this information with radio luminosities, we classify 92 per cent of the radio sources as a star-forming galaxy, high/low-excitation radio galaxy, or radio-quiet AGN and study the population demographics as a function of 150 MHz flux density, luminosity, SFR, stellar mass, redshift and apparent $r$-band magnitude. Finally, we use Prospector SED fits to investigate the SFR$-$150 MHz luminosity relation for a sample of $\sim$$133,000~3.6~\mu$m-selected $z<1$ sources, finding that the stellar mass dependence is significantly weaker than previously reported, and may disappear altogether at $\log_{10} (\mathrm{SFR}/M_\odot~\mathrm{yr}^{-1}) > 0.5$. This approach makes it significantly easier to classify radio sources from LoTSS and elsewhere, and may have important implications for future studies of star-forming galaxies at radio wavelengths.

==> adsjournals.tex <==
% define all the journal names from ADS

 \newcommand{\aj} { Astronomical Journal} 
 \newcommand{\actaa} { Acta Astronomica} 
 \newcommand{\araa} { Annual Review of Astron and Astrophys} 
 \newcommand{\apj} { Astrophysical Journal} 
 \newcommand{\apjl} { Astrophysical Journal, Letters} 
 \newcommand{\apjs} { Astrophysical Journal, Supplement} 
 \newcommand{\ao} { Applied Optics} 
 \newcommand{\apss} { Astrophysics and Space Science} 
 \newcommand{\aap} { Astronomy and Astrophysics} 
 \newcommand{\aapr} { Astronomy and Astrophysics Reviews} 
 \newcommand{\aaps} { Astronomy and Astrophysics, Supplement} 
 \newcommand{\azh} { Astronomicheskii Zhurnal} 
 \newcommand{\baas} { Bulletin of the AAS} 
 \newcommand{\caa} { Chinese Astronomy and Astrophysics} 
 \newcommand{\cjaa} { Chinese Journal of Astronomy and Astrophysics} 
 \newcommand{\icarus} {Icarus} 
 \newcommand{\jcap} { Journal of Cosmology and Astroparticle Physics} 
 \newcommand{\jrasc} { Journal of the RAS of Canada} 
 \newcommand{\memras} {Memoirs of the RAS} 
 \newcommand{\mnras} { Monthly Notices of the RAS} 
 \newcommand{\na} { New Astronomy} 
 \newcommand{\nar} { New Astronomy Review} 
 \newcommand{\pra} { Physical Review A: General Physics} 
 \newcommand{\prb} { Physical Review B: Solid State} 
 \newcommand{\prc} { Physical Review C} 
 \newcommand{\prd} { Physical Review D} 
 \newcommand{\pre} { Physical Review E} 
 \newcommand{\prl} { Physical Review Letters} 
 \newcommand{\pasa} { Publications of the Astron. Soc. of Australia} 
 \newcommand{\pasp} { Publications of the ASP} 
 \newcommand{\pasj} { Publications of the ASJ} 
 \newcommand{\rmxaa} { Revista Mexicana de Astronomia y Astrofisica} 
 \newcommand{\qjras} { Quarterly Journal of the RAS} 
 \newcommand{\skytel} {Sky and Telescope} 
 \newcommand{\solphys} {Solar Physics} 
 \newcommand{\sovast} {Soviet Astronomy} 
 \newcommand{\ssr} { Space Science Reviews} 
 \newcommand{\zap} { Zeitschrift fuer Astrophysik} 
 \newcommand{\nat} { Nature} 
 \newcommand{\iaucirc} {IAU Cirulars} 
 \newcommand{\aplett} {Astrophysics Letters} 
 \newcommand{\apspr} { Astrophysics Space Physics Research} 
 \newcommand{\bain} { Bulletin Astronomical Institute of the Netherlands} 
 \newcommand{\fcp} { Fundamental Cosmic Physics} 
 \newcommand{\gca} { Geochimica Cosmochimica Acta} 
 \newcommand{\grl} { Geophysics Research Letters} 
 \newcommand{\jcp} { Journal of Chemical Physics} 
 \newcommand{\jgr} { Journal of Geophysics Research} 
 \newcommand{\jqsrt} { Journal of Quantitiative Spectroscopy and Radiative Transfer} 
 \newcommand{\memsai} {Mem. Societa Astronomica Italiana} 
 \newcommand{\nphysa} {Nuclear Physics A} 
 \newcommand{\physrep} {Physics Reports} 
 \newcommand{\physscr} {Physica Scripta} 
 \newcommand{\planss} {Planetary Space Science} 
 \newcommand{\procspie} {Proceedings of the SPIE}
